On the growth of iterated monodromy groups

Nekrashevych conjectured that the iterated monodromy groups of quadratic polynomials with preperiodic critical orbit have intermediate growth. We illustrate some of the difficulties that arise in attacking this conjecture and prove subexponential growth for the iterated monodromy group of $z^2+i$. This is the first non-trivial example supporting the conjecture.

==> basic_notation.tex <==
%% LaTeX2e file `basic_notation.tex'
%% generated by the `filecontents' environment
%% from source `growth_of_iterated_monodromy_groups' on 2004/05/17.
%%
\ProvidesFile{basic_notation.tex}[2001/09/20 KUB]

%
% This should be merged with buxmath.sty at some point
%

\newcommand{\congruent}{\equiv}


\newcommand{\DisplayOrList}[1]{%
  \ifNotationlisting
    \(#1\)%
  \else
    \[#1\]%
  \fi
}

%
% labelling defining occurences
%
\newcommand{\defnotion}[1]{%
  \begingroup
%    \def\tmp{#1}%
%    \expandafter\label\expandafter{\meaning\tmp}%
    \notion{#1}%
  \endgroup
}
\newcommand{\defref}[1]{%
  \begingroup
    \def\tmp{#1}%
    \expandafter\ref\expandafter{\meaning\tmp}%
  \endgroup
}
\newcommand{\defpref}[1]{%
  (\defref{#1})%
}
\newcommand{\locnotion}[1]{\emph{#1}}

%
% vertical =
%
\newcommand{\veq}{\shortparallel}

%
% set theory
%

\newcommand{\union}{\cup\OptIndex}
\newcommand{\symmetricdifference}{\mathbin{\triangle}}%{\mathbin{+_\Two}}
\newcommand{\intersect}[1][]{\cap_{#1}}
%\newcommand{\disjointunion}{\,\,\hbox to 0pt{$\hss\cdot\hss$}\hbox to 0pt{$\hss\union\hss$}\,\,}
\newcommand{\disjointunion}{\uplus}
\newcommand{\equalls}[1][]{%
  \IfEmptyThenElse{#1}{%
    =
  }{%
    =_{#1}
  }
}

\newcommand{\Parentheses}[1]{\left(#1\right)}
\newcommand{\Brakets}[1]{\left[#1\right]}
\newcommand{\ToThePower}[2]{#1^{#2}}
\newcommand{\AbsValue}[1]{\left|#1\right|}
\newcommand{\Factorial}[1]{#1!}

\newcommand{\EvalAt}{\negthinspace\Parentheses}
\newcommand{\ImageAt}{\negthinspace\Parentheses}
\newcommand{\ActOn}{\cdot}
\newcommand{\RestrictionTo}[1]{|_{#1}}

\newcommand{\OpenInterval}[2]{\left(#1,#2\right)}
\newcommand{\ClosedInterval}[2]{\left[#1,#2\right]}
\newcommand{\RightOpenInterval}[2]{\left[#1,#2\right)}
\newcommand{\LeftOpenInterval}[2]{\left(#1,#2\right]}

\newcommand{\Binom}[2]{\left(\begin{array}{c}#1\\#2\end{array}\right)}

\newcommand{\gobbleopt}[1][]{}

\newcommand{\forinf}{\exists^\infty}
\newcommand{\Forsome}[1]{\text{\ for some\ }#1}
\newcommand{\Forall}[1]{\text{\ for all\ }#1}
\newcommand{\Forinfmany}[1]{\qquad\text{\ for infinitely many\ }#1}
\newcommand{\ForSome}[1]{\qquad\text{\ for some\ }#1}
\newcommand{\ForAll}[1]{\qquad\text{\ for all\ }#1}
\newcommand{\ForInfMany}[1]{\qquad\text{\ for infinitely many\ }#1}
\newcommand{\For}[1]{\qquad\text{\ for\ }#1}
\newcommand{\Since}[1]{\qquad\text{\ since\ }#1}
\newcommand{\With}[1]{\qquad\text{\ with\ }#1}
\newcommand{\As}[1]{\qquad\text{\ as\ }#1}
\newcommand{\AND}{\qquad\text{\ and\ }\qquad}
%\newcommand{\OR}{\qquad\text{\ or\ }\qquad}
%\newcommand{\IF}{\qquad\text{\ if\ }\qquad}
\newcommand{\IFF}{\qquad\text{\ if and only if\ }\qquad}
\newcommand{\DefIff}{:\Longleftrightarrow}
\newcommand{\Iff}{\ensuremath{\Longleftrightarrow}}
\newcommand{\Implies}{\ensuremath{\Longrightarrow}}

\newcommand{\ExtPowerOf}[2][]{%
  \ExtPot^{#1}\left(#2\right)
}
\newcommand{\tensor}[1][]{\otimes_{#1}}
\newcommand{\BilOf}[2][]{%
  \operatorname{Bil}_{#1}\negthinspace\left(#2\right)
}
\newcommand{\ExpOf}[2][]{\mathop{\exp_{#1}}\negthinspace\left(#2\right)}

\newcommand{\Diff}[1]{\mathrm{d}#1}
\newcommand{\Brace}[3]{%
  \left[#3\right]_{#1}^{#2}
}

\newcommand{\mapcolon}{:}

%
% Compound Notations
%
\makeatletter
\newcommand{\TwoByTwoMatrix}[4]{%
    \left(\begin{array}{cc}
      #1 & #2\\
      #3 & #4
    \end{array}\right)
}

\newcommand{\TwoByTwoDet}[4]{%
    \left|\begin{array}{cc}
      #1 & #2\\
      #3 & #4
    \end{array}\right|
}

\newcommand{\TwoColVector}[2]{%
    \left(\begin{array}{cc}
      #1\\
      #2
    \end{array}\right)
}

\newcommand{\TwoRwoVector}[2]{%
  \Parentheses{#1,#2}
}
\providecommand{\IfEmptyThenElse}[1]{%
  \begingroup
    \def\tempa{#1}%
    \def\tempb{}%
    \ifx\tempa\tempb
      \def\next{\@firstoftwo}%
    \else
      \def\next{\@secondoftwo}%
    \fi
  \expandafter\endgroup\next
}

\newcommand{\getfamfirstarg}[1][]{
  \def\tempa{#1}%
  \getfamsecondarg
}
\newcommand{\getfamsecondarg}[2][]{
  \def\tempb{#1}%
  \def\empty{}%
  \ifx\tempa\empty
    \left(#2\right)%
  \else
    \ifx\tempb\empty
      \left(#2\right)_{\tempa}%
    \else
      \left(#2\right)_{\tempa}^{\tempb}%
    \fi
  \fi
  \endgroup
}
\newcommand{\FamOf}{%
  \begingroup
    \getfamfirstarg
}
\iffalse
\newcommand{\FamOf}[2][]{%
  \IfEmptyThenElse{#1}{
    \left(#2\right)
  }{
    \left(#2\right)_{#1}
  }
}
\fi

\newcommand{\SetOf}[2][]{%
  \IfEmptyThenElse{#1}{
    \left\{#2\right\}
  }{
    \left\{#1\,\,\vrule\,\,#2\right\}
  }
}

\newcommand{\GroupPresented}[2][]{%
  \IfEmptyThenElse{#1}{
    \left\langle#2\right\rangle
  }{
    \left\langle#1\,\,\vrule\,\,#2\right\rangle
  }
}
\newcommand{\EquivClassOf}[2][]{\left[#2\right]_{#1}}
\newcommand{\TupelOf}[2][]{\left(#2\right)_{#1}}
\newcommand{\MaxOf}[2][]{%
  \IfEmptyThenElse{#1}{
    \max\left(#2\right)
  }{
    \max_{#1}\left(#2\right)
  }
}

\newcommand{\MinOf}[2][]{%
  \IfEmptyThenElse{#1}{
    \min\left(#2\right)
  }{
    \min_{#1}\left(#2\right)
  }
}

\newcommand{\InitTripleCommand}[2][]{%
  \begingroup
    \def\EndSymbol{#1}
    \def\TheSymbol{#2}%
    \getfirstarg
}
\newcommand{\getfirstarg}[1][]{%
    \def\tempa{#1}%
    \getlastargs
  }
\newcommand{\getlastargs}[2][]{%
    \def\tempb{#1}%
    \def\empty{}%
    \ifx\tempb\empty
      \ifx\tempa\empty
        \TheSymbol #2%
      \else
        \TheSymbol_{\tempa}#2%
      \fi
    \else
      \TheSymbol_{\tempa}^{#1}#2%
    \fi
  \endgroup
}

\newcommand{\Lim}[2][]{\lim_{#1}#2}

\newcommand{\Sum}[0]{\InitTripleCommand{\sum}}
\newcommand{\Int}[0]{\InitTripleCommand{\int}}
\newcommand{\Union}[0]{\InitTripleCommand{\bigcup}}
\newcommand{\Intersection}[0]{\InitTripleCommand{\bigcap}}
\newcommand{\DisUnion}[0]{\InitTripleCommand{{\biguplus}}}
\newcommand{\Product}[0]{\InitTripleCommand{\prod}}
\newcommand{\CoProduct}[0]{\InitTripleCommand{\coprod}}
\newcommand{\XProduct}[0]{\InitTripleCommand{\bigtimes}}
\newcommand{\FreeProd}[0]{\InitTripleCommand{\bigast}}
\newcommand{\BigJoin}[0]{\InitTripleCommand{\bigast}}
\newcommand{\DirectSum}[0]{\InitTripleCommand{\bigoplus}}
\newcommand{\Min}[0]{\InitTripleCommand{\min}}
\newcommand{\Max}[0]{\InitTripleCommand{\max}}
\newcommand{\Inf}[0]{\InitTripleCommand{\inf}}
\newcommand{\InfOf}[2][]{%
  \IfEmptyThenElse{#1}{
    \inf#2
  }{
    \inf_{#1}#2
  }
}
\newcommand{\Sup}[0]{\InitTripleCommand{\sup}}
\newcommand{\SupOf}{\sup}

\newcommand{\MatrixOf}[2][]{%
  \IfEmptyThenElse{#1}{%
    \left(#2\right)
  }{%
    \left(#2\right)_{#1}
  }
}

\newcommand{\OrderOf}{\operatorname{ord}\OptIndexParentheses}

\newcommand{\TensorProduct}[3][]{%
  \IfEmptyThenElse{#1}{
    #2\otimes#3
  }{
    #2\otimes_{#1}#3
  }
}

\newcommand{\leftsemidirectprod}[1][]{%
  \rtimes\OptIndex[#1]
}

\newcommand{\wreathprod}{\wr}

\newcommand{\ColumnVector}[1]{%
  \left(\begin{array}{c}
    #1
  \end{array}\right)
}

\newcommand{\Interval}[2]{\left[#1,#2\right]}

% \makeatletter
% \def\@lap[#1,#2]#3{%
%   \parbox[b][0pt][b]{0pt}{%
%     \raisebox{#2}{%
%       \parbox[b][0pt][c]{0pt}{%
%          \makebox[0pt][c]{\null\kern#1\kern#1{#3}}%
%       }%
%     }%
%   }%
%   \ignorespaces
% }%
% \newcommand{\clap}[2][0pt,0pt]{\@lap[#1]{#2}}
% \makeatother

\newcommand{\clap}[1]{\makebox[0pt][c]{#1}}


\newcommand{\PreImage}[2]{{#1}^{-1}\left(#2\right)}
%
%
%
\newcommand{\IfNonEmpty}[2]{\IfEmptyThenElse{#1}{}{#2}}
\newcommand{\OptExponent}[1][]{\IfNonEmpty{#1}{^{#1}}}
\newcommand{\OptParExponent}[1][]{\IfNonEmpty{#1}{^{\left(#1\right)}}}
\newcommand{\OptIndex}[1][]{\IfNonEmpty{#1}{_{#1}}}
\newcommand{\OptArg}[2]{#1\IfNonEmpty{#2}{\EvalAt{#2}}}
\newcommand{\OptIndexOptPar}[1][]{\IfNonEmpty{#1}{_{#1}}\OptParentheses}
\newcommand{\OptParentheses}[1][]{\IfNonEmpty{#1}{\negthinspace\left(#1\right)}}
\newcommand{\OptExponentParentheses}[1][]{\IfNonEmpty{#1}{^{#1}}\EvalAt}
\newcommand{\OptIndexParentheses}[1][]{\IfNonEmpty{#1}{_{#1}}\OptExponentParentheses}
\newcommand{\OptIndexParExponent}[1][]{\IfNonEmpty{#1}{_{#1}}\OptParExponent}
\newcommand{\OptIndexExponent}[1][]{\IfNonEmpty{#1}{_{#1}}\OptExponent}
\newcommand{\DoubleArg}[2]{\EvalAt{#1,#2}}
\newcommand{\OptExponentDoubleArg}[1][]{\IfNonEmpty{#1}{_{#1}}\DoubleArg}
\newcommand{\OptIndexDoubleArg}[1][]{\IfNonEmpty{#1}{_{#1}}\OptExponentDoubleArg}
\newcommand{\newconst}[2]{%
  \newcommand{#1}[0]{#2}
  }
\newcommand{\UnVar}[1]{%
  \let#1\undefined
  \expandafter\let\csname\expandafter\@gobble\string#1Of\endcsname\undefined
}
\newcommand{\newvariable}[2]{%
  \newcommand{#1}[1][]{#2\IfNonEmpty{##1}{_{##1}}\OptExponent}
  \expandafter\newcommand\csname\expandafter\@gobble\string#1Of\endcsname{#1\OptIndexParentheses}
  }
\newcommand{\renewvariable}[2]{%
  \renewcommand{#1}[1][]{#2\IfNonEmpty{##1}{_{##1}}\OptExponent}
  \expandafter\renewcommand\csname\expandafter\@gobble\string#1Of\endcsname{#1\OptIndexParentheses}
  }
\newcommand{\tmpvariable}[2]{%
  \let#1\undefined
  \expandafter\let\csname\expandafter\@gobble\string#1Of\endcsname\undefined
  \newcommand{#1}[1][]{#2\IfNonEmpty{##1}{_{##1}}\OptExponent}
  \expandafter\newcommand\csname\expandafter\@gobble\string#1Of\endcsname{#1\OptIndexParentheses}
  }
\newcommand{\newparexpvariable}[2]{%
  \newcommand{#1}{#2\OptIndexParExponent}
  }
\newcommand{\newmap}[2]{%
  \newcommand{#1}[1][]{\OptArg{#2}{##1}}
  }
\newcommand{\newindexedmap}[2]{%
  \newcommand{#1}[1][]{#2\IfNonEmpty{##1}{_{##1}}\OptParentheses}
  }
\newcommand{\NewMap}[2]{%
  \newvariable{#1}{#2}%
  \begingroup
    \escapechar=-1%
    \expandafter\global\expandafter\newcommand\expandafter{\csname \string#1Of\endcsname}{#2\OptIndexParentheses}
  \endgroup
}
\newcommand{\newMap}[2]{%
  \newcommand{#1}[1][]{#2\IfNonEmpty{##1}{_{##1}}\EvalAt}
  }
\newcommand{\newMapTwo}[2]{%
  \newcommand{#1}[2]{#2\left(##1,##2\right)}
  }
\newcommand{\newMapTWO}[2]{%
  \newcommand{#1}[2]{#2\left(##1;##2\right)}
  }
\newcommand{\newexpvector}[2]{%
  \newcommand{#1}{#2\OptParExponent}
  }

\newcommand{\newexpvar}[2]{%
  \newcommand{#1}{#2\OptIndexExponent}
}
\newcommand{\newparexpvar}[2]{%
  \newcommand{#1}{#2\OptIndexParExponent}
}
\newcommand{\OR}{\quad\text{or}\quad}
%
% picture
%
  \newcommand{\drawpath}[1]{%
    \begingroup%
      \edef\tempa{#1}%
      \expandafter\drawline\tempa%
    \endgroup%
    \ignorespaces
  }
  \newcommand{\dashpath}[2]{%
    \begingroup%
      \edef\tempa{#2}%
      \def\tempb{\dashline[0]{#1}}%
      \expandafter\tempb\tempa%
    \endgroup%
    \ignorespaces
  }
  \newcommand{\plot}[2]{%
    \expandafter\put#1{#2}\ignorespaces
  }
  \def\lap[#1,#2]#3{%
    \parbox[b][0pt][b]{0pt}{%
      \raisebox{#2}{%
        \parbox[b][0pt][c]{0pt}{%
           \makebox[0pt][c]{\null\kern#1\kern#1{#3}}%
        }%
      }%
    }%
    \ignorespaces
  }%
  \newcommand{\Bullet}[2][0mm,0mm]{%
    \lap[0mm,0mm]{$\bullet$}
    \lap[#1]{$#2$}
  }

\newcommand{\UnitsOf}[1]{#1^{*}}
\newcommand{\ThePullback}[1]{#1^{*}\OptParentheses}

\newcommand{\DirectedSystem}[3][]{%
  \IfEmptyThenElse{#1}{%
    (#2)_{#3}
  }{%
    (#2)_{#1\in#3}%
  }%
}

\newcommand{\Morph}[3][]{%
  \IfEmptyThenElse{#1}{%
    \mathop{\mathrm{Mor}}\left(#2,#3\right)%
  }{%
    \mathop{\mathrm{Mor}}\limits_{#1}\left(#2,#3\right)%
  }%
}
\newcommand{\InvLimit}[2][]{\mathop{\inverslim}_{#1}#2}
\newindexedmap{\InvLimitMap}{\pi}
\newmap{\InvUnivMap}{\iota}
\newcommand{\DirLimit}[2][]{\mathop{\directlim}_{#1}#2}
\newindexedmap{\DirLimitMap}{\iota}
\newmap{\DirUnivMap}{\pi}
\newcommand{\Limit}[2][]{\mathop{\lim}_{#1}#2}

\newcommand{\HoColimOf}[1]{%
  \operatorname{ho-colim}\left(#1\right)
}

\newcommand{\FunctorMap}[1]{#1_{*}\OptParentheses}
\newvariable{\TheGraphLift}{\tilde{\TheGraph}}
\newcommand{\graphminus}{-}
\newvariable{\TheEdgeLift}{\tilde{\TheEdge}}

%
% small integers
%
\newcommand{\Number}[1]{#1}
\newvariable{\Zero}{\Number{0}}
\newvariable{\One}{\Number{1}}
\newvariable{\qOne}{1}
\newvariable{\OneHalf}{\ensuremath{\frac{1}{2}}}
\newvariable{\Two}{\Number{2}}
\newvariable{\Three}{\Number{3}}
\newvariable{\Four}{\Number{4}}
\newvariable{\Five}{\Number{5}}
\newvariable{\Six}{\Number{6}}
\newvariable{\Seven}{\Number{7}}
\newvariable{\Eight}{\Number{8}}
\newvariable{\Nine}{\Number{9}}
\newvariable{\Ten}{\Number{10}}


%
% Group Actions
%
\newcommand{\ActingOn}{\negthinspace.}
\newcommand{\ActsOn}{\curvearrowright}

\endinput


==> bibliography.tex <==
%% LaTeX2e file `bibliography.tex'
%% generated by the `filecontents' environment
%% from source `growth_of_iterated_monodromy_groups' on 2004/05/17.
%%
\ProvidesFile{bibliography.tex}[2001/10/16 KUB]
\newcommand{\nametie}{\,}
\begin{references}%
  \newcommand{\BielPre}[2]{%
    Preprint series #1 -- #2, SFB~343; Bielefeld (19#1)%
  }%
  \begin{article}{Abel79}{Abels:1979}%
    \au{H.\nametie Abels}
    \ti{An example of a finitely presented solvable group}
    \lo{In \cite{Wall:1979}}{205 -- 211}
  \end{article}
  \begin{book}{Abel87}{Abels:1987}%
    \au{H.\nametie Abels}
    \ti{Finite presentability of $S$-arithmetic groups -- Compact
        presentability of solvable groups}
    \lo{Springer LNM~1261 (1987)}{}
  \end{book}
  \begin{article}{Abel91}{Abels:1991}
    \au{H.\nametie Abels}
    \ti{Finiteness Properties of certain arithmetic groups in the function field case}
    \lo{Israel J.\ Math.\ 76 (1991)}{113 -- 128}
  \end{article}
  \begin{article}{AbBr87}{Abels.Brown:1987}
    \au{H.\nametie Abels, K.S.\nametie Brown}
    \ti{Finiteness Properties of Solvable $S$-Arithmetic Groups: An Example}
    \lo{Journal of Pure and Applied Algebra 44 (1987)}{77 -- 83}
  \end{article}
  \begin{article}{AbHo93}{Abels.Holz:1993}
    \au{H.\nametie Abels, S.\nametie Holz}
    \ti{Higher Generation by Subgroups}
    \lo{Journal of Algebra 160 (1993)}{310 -- 341}
  \end{article}
  \begin{article}{AbTi97}{Abels.Tiemeyer:1997}%
    \au{H.\nametie Abels, A.\nametie Tiemeyer}
    \ti{Compactness Properties of Locally Compact Groups}
    \lo{Transformation Groups 2 (1997)}{119 - 135}
%    (confer~\cite{Tiemeyer:1997})
  \end{article}
  \begin{article}{\AA{}ber86}{Aberg:1986}%
    \au{H.\nametie \AA{}berg}
    \ti{Bieri-Strebel Valuations (of Finite Rank)}
    \lo{Proceedings of the London Mathematical Society 52 (1986)}{269 -- 304}
  \end{article}
  \begin{article}{Abra95}{Abramenko:review:1995}
    \au{P.\nametie Abramenko}
    \ti{Review 95e:20049 on \cite{Abels.Holz:1993}}
    \lo{Mathematical Reviews (1995)}{}
  \end{article}
  \begin{thesis}{Abra87}{Abramenko:1987}
    \au{P.\nametie Abramenko}
    \ti{Endlichkeitseigenschaften der Gruppen $\SL_n(\FFF_q[t])$}
    \lo{Thesis Frankfurt am Main (1987)}{}
  \end{thesis}
  \begin{notes}{Abra94}{Abramenko:1994}
    \au{P.\nametie Abramenko}
    \ti{{\selectlanguage{german}Chevalleygruppen}}
    \lo{Manuscript (Frankfurt, WS~1994/95)}{}
  \end{notes}
  \begin{thesis}{Abra95}{Abramenko:1995}%
    \au{P.\nametie Abramenko}
    \ti{Twin Buildings, Spherical buildings and Finiteness
        Properties of Almost Simple $\FFF_q$-Groups over
        $\FFF_q[t]$}
    \lo{Habilitation thesis (Frankfurt, 1995)}{}
  \end{thesis}
  \begin{book}{Abra96}{Abramenko:1996}%
    \au{P.\nametie Abramenko}
    \ti{Twin Buildings and Applications to $S$-Arithmetic Groups}
    \lo{Springer LNM~1641 (1996)}{}
  \end{book}
  \begin{preprint}{Abra99}{Abramenko:unpublished}
    \au{P.\nametie Abramenko}
    \ti{??}
    \lo{??}{}
  \end{preprint}
  \begin{article}{Akit01}{Akita:2001}
    \au{T.\nametie Akita}
    \ti{Homological infiniteness of Torelli groups}
    \lo{Topology 40 (2001), no. 2}{213 -- 221}
  \end{article}
  \begin{article}{Alon94}{Alonso:1994}
    \au{J.\nametie Alonso}
    \ti{Finiteness conditions on groups and quasi-isometries}
    \lo{Journal of Pure and Applied Algebra 95 (1994)}{121 -- 129}
  \end{article}
  \begin{book}{Alpe91}{Alperin:1991}
    \ed{R.\nametie Alperin}
    \ti{Arboreal Group Theory}
    \lo{MSRI Publications 19 (Springer, 1991)}{}
  \end{book}
  \begin{article}{BBLSW99}{Babson.Bjoerner.Linusson.Shareshian.Welker:1999}%
    \au{E.\nametie Babson, A.\nametie Bj\"{o}rner, S.\nametie Linusson, J.\nametie Shareshian, V.\nametie Welker}
    \ti{Complexes of Not $i$-Connected Graphs}
    \lo{Topology 38(2) (1999)}{271 -- 299}
  \end{article}
  \begin{preprint}{Bart00}{Bartholdi:2000}
    \au{L.\nametie Bartholdi}
    \ti{The growth of Grigorchuk's group}
    \lo{preprint (2000) arXiv:math.GR/0012108}{}
  \end{preprint}
  \begin{preprint}{BGN02}{Bartholdi.Grigorchuk.Nekrashevych:2002}%
    \au{L.\nametie Bartholdi, R.I.\nametie Grigorchuk, V.\nametie Nekrashevych}
    \ti{From Fractal Groups to Fractal Sets}
    \lo{preprint (2002) arXiv:math.GR/0202001v4}{}
  \end{preprint}
  \begin{preprint}{BGS01}{Bartholdi.Grigorchuk.Sunik:2001}%
    \au{L.\nametie Bartholdi, R.I.\nametie Grigorchuk, Z.\nametie \v{S}uni\'{k}}
    \ti{Branch Groups}
    \lo{preprint (2001)}{}
  \end{preprint}
  \begin{article}{BBN59}{Baumslag.Boone.Neumann:1959}%
    \au{G.\nametie Baumslag, W.W.\nametie Boone, B.H.\nametie Neumann}
    \ti{Some Unsolvable Problems About Elements and Subgroups of Groups}
    \lo{Mathematica Scandinavica 7 (1959)}{191 -- 201}
  \end{article}
  \begin{article}{Behr62}{Behr:1962}%
    \au{H.\nametie Behr}
    \ti{{\selectlanguage{german}\"U{}ber die endliche Definierbarkeit von Gruppen}}
    \lo{{\selectlanguage{german}Journal f\"u{}r die reine und angewandte
        Mathematik (Crelles Journal) 211 (1962)}}{116 -- 122}
  \end{article}
  \begin{article}{Behr68}{Behr:1968}%
    \au{H.\nametie Behr}
    \ti{{\selectlanguage{german}Zur starken Approximation in algebraischen Gruppen \"u{}ber globalen
        K\"o{}rpern}}
    \lo{{{\selectlanguage{french}Journal f\"u{}r die reine und angewandte
        Mathematik (Crelles Journal) 229 (1968)}}}{107 -- 116}
  \end{article}
  \begin{preprint}{Behr98}{Behr:1998}%
    \au{H.\nametie Behr}
    \ti{Arithmetic groups over function fields I\null.
        A complete
        characterization of finitely generated and finitely presented
        arithmetic subgroups of reductive algebraic groups}
    \lo{{\selectlanguage{german}Journal f\"u{}r die reine und
        angewandte Mathematik (Crelles Journal) 495 (1998)}}{79--118}
  \end{preprint}
  \begin{preprint}{Behr99}{Behr:1999}
    \au{H.\nametie Behr}
    \ti{Higher finiteness properties of $S$-arithmetic groups in the function field case I: Chevalley groups with coefficients in $\FFF_q[t]$}
    \lo{Preprint, Frankfurt (1999)}{}
  \end{preprint}
  \begin{preprint}{BeBr03}{Belk.Brown:2003}
    \au{J.M.\nametie Belk, K.S.\nametie Brown}
    \ti{Forest Diagrams for Elements of Thompson's Group $F$}
    \lo{Preprint (2003), arXiv:math.GR/0305412}{}
  \end{preprint}
  \begin{preprint}{BeBu02a}{Belk.Bux:2002a}
    \au{J.M.\nametie Belk, K.-U.\nametie Bux}
    \ti{Flows, Robots, and Amenability} % A Max-Flow-Min-Cut Theorem for Infinite Graphs and Applications to Amenability}
    \lo{Preprint in preparation}{}
  \end{preprint}
  \begin{preprint}{BeBu02b}{Belk.Bux:2002b}
    \au{J.M.\nametie Belk, K.-U.\nametie Bux}
    \ti{Thompson's Group $F$ is not Minimally Almost Convex}
    \lo{Preprint in preparation}{}
  \end{preprint}
  \begin{preprint}{BeBu03}{Belk.Bux:2003}
    \au{J.M.\nametie Belk, K.-U.\nametie Bux}
    \ti{Thompson's Group $F$ is not Minimally Almost Convex}
    \lo{Preprint, arXiv:math.GR/0301141}{}
  \end{preprint}
  \begin{preprint}{BeBu02c}{Belk.Bux:2002c}
    \au{J.M.\nametie Belk, K.-U.\nametie Bux}
    \ti{A Series of Groups Related to Thompson's Groups $F$ and $T$}
    \lo{Preprint in preparation}{}
  \end{preprint}
  \begin{article}{BeBr97}{Bestvina.Brady:1997}%
    \au{M.\nametie Bestvina, N.\nametie Brady}
    \ti{Morse theory and finiteness properties of groups}
    \lo{Inventiones mathematicae 129 (1997)}{445 -- 470}
  \end{article}
  \begin{article}{BeFe00}{Bestvina.Feighn:2000}
    \au{M.\nametie Bestvina, M.\nametie Feighn}
    \ti{The topology at infinity of $\Out(F_n)$}
    \lo{Inventiones mathematicae 140 (2000)}{651 -- 692}
  \end{article}
  \begin{article}{BFH00a}{Bestvina.Feighn.Handel:2000a}
    \au{M.\nametie Bestvina, M.\nametie Feighn, M.\nametie Handel}
    \ti{The Tits Alternative for $\operatorname{Out}(F_n)$ I: Dynamics of exponentially growing automorphisms}
    \lo{Annals of Mathematics 151 (2000)}{517 -- 623}
  \end{article}
  \begin{preprint}{BFH00b}{Bestvina.Feighn.Handel:2000b}
    \au{M.\nametie Bestvina, M.\nametie Feighn, M.\nametie Handel}
    \ti{The Tits Alternative for $\operatorname{Out}(F_n)$ II: A Kolchin Theorem}
    \lo{preprint}{}
  \end{preprint}
  \begin{article}{Bier99}{Bieri:1999}%
    \au{R.\nametie Bieri}
    \ti{Finiteness length and connectivity length for groups}
    \lo{In \cite{Cossey.Miller.Neumann.Shapiro:1999}}
         {9 -- 22}
  \end{article}
  \begin{article}{BiEc74}{Bieri.Eckmann:1974}
    \au{R.\nametie Bieri, B.\nametie Eckmann}
    \ti{Finiteness Properties of Duality Groups}
    \lo{Commentarii Mathematici Helvetici 49 (1974)}{74 -- 83}
  \end{article}
  \begin{preprint}{BiGe98}{Bieri.Geoghegan:1998}%
    \au{R.\nametie Bieri, R.\nametie Geoghegan}
    \ti{Connectivity properties of group actions on non-positively
        curved spaces~II: The geometric invariants}
    \lo{Preprint (Frankfurt, October~1998)}{}
  \end{preprint}
  \begin{preprint}{BiHa00}{Bieri.Harlander:2000}
    \au{R.\nametie Bieri, J.\nametie Harlander}
    \ti{On the FP$_3$-Conjecture for Metabelian Groups}
    \lo{Preprint (Frankfurt, 2000)}{}
  \end{preprint}
  \begin{article}{BiRe88}{Bieri.Renz:1988}%
    \au{R.\nametie Bieri, B.\nametie Renz}
    \ti{Valuations on free resolutions and higher geometric
        invariants of groups}
    \lo{Commentarii Mathematici Helvetici 63 (1988)}{464 -- 497}
  \end{article}
  \begin{article}{BiSt80}{Bieri.Strebel:1980}
    \au{R.\nametie Bieri, R.\nametie Strebel}
    \ti{Valuations and Finitely Presented Metabelian Groups}
    \lo{Proceedings of the London Mathematical Society 41 (1980)}{439 -- 464}
  \end{article}
  \begin{manuscript}{BiSt}{Bieri.Strebel:nodate}
    \au{R.\nametie Bieri, R.\nametie Strebel}
    \ti{On Groups of PL-Homemorphisms of the Real Line}
    \lo{Unpublished Manuscript}{}
  \end{manuscript}
  \begin{preprint}{BiSt92}{Bieri.Strebel:1992}
    \au{R.\nametie Bieri, R.\nametie Strebel}
    \ti{Geometric Invariants of Discrete Groups}
    \lo{Preprint (Frankfurt, 1992)}{}
  \end{preprint}
  \begin{article}{Bj\"{o}r92}{Bjoerner:1992}
    \au{A.\nametie Bj\"orner}
    \ti{The Homology and Shellability of Matroids and Geometric Lattices}
%    \lo{in \ed{N.\nametie White (ed.)} \ti{Matroid Applications}
%        (Cambridge University Press 1992)}{ 226 -- 283}
    \lo{In \cite{White:1992}}{226 -- 283}
  \end{article}
  \begin{article}{BLVZ94}{Bjoerner.Lovasz.Vrecica.Zivaljevic:1994}%
    \au{A.\nametie Bj\"orner, L.\nametie Lov\'{a}sz, S.T.\nametie Vre\'{c}ica, R.T.\nametie \v{Z}ivaljevi\'{c}}
    \ti{Chessboard complexes and matching complexes}
    \lo{Journal of the London Mathematical Society 49 (1994)}{25 -- 39}
  \end{article}
  \begin{article}{Bore62}{Borel:1962}%
    \au{A.\nametie Borel}
    \ti{Arithmetic properties of linear algebraic groups}
    \lo{Proceeding of the International Congress of Mathematicians, Stockholm, 1962
        (Upsala 1963)}{10 -- 22}
  \end{article}
  \begin{article}{Bore63}{Borel:1963}%
    \au{A.\nametie Borel}
    \ti{Some finiteness properties of adele groups over number fields}
    \lo{Publ.\ Math., Inst.\ Hautes Etud.\ Sci.\ 16 (1963)}{5 -- 30}
  \end{article}
  \begin{book}{Bore91}{Borel:1991}%
    \au{A.\nametie Borel}
    \ti{Linear Algebraic Groups}
    \edition{Second Enlarged Edition}
    \lo{Springer GTM 126, New York (1991)}{}
  \end{book}
  \begin{article}{BoHa62}{Borel.Harish-Chandra:1962}%
    \au{A.\nametie Borel, Harish-Chandra}
    \ti{Arithmetic subgroups of algebraic groups}
    \lo{Annals of Mathematics 75 (1962)}{485 -- 535}
  \end{article}
  \begin{article}{BoSe73}{Borel.Serre:1973}%
    \au{A.\nametie Borel, J-P.\nametie Serre}
    \ti{Corners and arithmetic groups}
    \lo{Commentarii Mathematici Helvetici 48 (1973)}{436 -- 491}
  \end{article}
  \begin{article}{BoSe76}{Borel.Serre:1976}%
    \au{A.\nametie Borel, J.-P.\nametie Serre}
    \ti{{\selectlanguage{french}Cohomologie d'immeubles et de groupes S-arithm\'{e}tiques}}
    \lo{Topology 15 (1976)}{211 -- 232}
  \end{article}
  \begin{article}{BoTi65}{Borel.Tits:1965}%
    \au{A.\nametie Borel, J.\nametie Tits}
    \ti{Groupes r\'{e}ductifs}
    \lo{Publ.\ Math., Inst.\ Hautes Etud.\ Sci.\ 27 (1965)}{55 -- 150}
  \end{article}
  \begin{article}{Brid00}{Bridson:2000}
    \au{M.\nametie Bridson}
    \ti{Finiteness Properties for Subgroups of $\GL(n,\ZZZ)$}
    \lo{Math. Annalen., 317 (2000)}{629 -- 633}
  \end{article}
  \begin{book}{BrHa99}{Bridson.Haefliger:1999}
    \au{M.R.\nametie Bridson, A.\nametie Haefliger}
    \ti{Metric Spaces of Non-Positive Curvature}
    \lo{{\selectlanguage{german}Grundlehren der Mathematischen Wissenschaften} (Springer, 1999)}{}
  \end{book}
  \begin{article}{BrVo01}{Bridson.Vogtmann:2001}
    \au{M.\nametie Bridson, K.\nametie Vogtmann}
    \ti{The symmetries of Outer space}
    \lo{Duke Mathematical Journal 106 (2001), no. 2}{391 -- 409}
  \end{article}
  \begin{book}{Brow82}{Brown:1982}%
    \au{K.S.\nametie Brown}
    \ti{Cohomology of Groups}
    \lo{Springer GTM 87, New York (1982)}{}
  \end{book}
  \begin{article}{Bro87a}{Brown:1987a}%
    \au{K.S.\nametie Brown}
    \ti{Finiteness Properties of Groups}
    \lo{Journal of Pure and Applied Algebra 44 (1987)}{45 -- 75}
  \end{article}
  \begin{article}{Bro87b}{Brown:1987b}%
    \au{K.S.\nametie Brown}
    \ti{Trees, valuations, and the Bieri-Neumann-Strebel invariant}
    \lo{Inventiones mathematicae 90 (1987)}{479 -- 504}
  \end{article}
  \begin{book}{Brow89}{Brown:1989}
    \au{K.S.\nametie Brown}
    \ti{Buildings}
    \lo{Springer, New York, Berlin (1989)}{}
  \end{book}
  \begin{article}{BrGe84}{Brown.Geoghegan:1984}%
    \au{K.S.\nametie Brown, R.\nametie Geoghegan}
    \ti{An infinite-dimensional torsion-free $FP_\infty$ group}
    \lo{Inventiones mathematicae 77 (1984)}{367 -- 381}
  \end{article}
  \begin{report}{BrTi72}{Bruhat.Tits:1972}%
    \au{F.\nametie Bruhat, J.\nametie Tits}
    \ti{{\selectlanguage{french}Groupes R\'{e}ductives sur un Corps Local I}}
    \lo{{\selectlanguage{french}Publications Math\'{e}matiques IHES 41 (1972)}}{5 -- 252}
  \end{report}
  \begin{article}{BBW79}{Brunner.Burns.Wiegold:1979}
    \au{A.M.\nametie Brunner, R.G.\nametie Burns, J.\nametie Wiegold}
    \ti{On the Number of Quotients, of One Kind or Another, of the Modular Group}
    \lo{Mathematical Scientist 4 (1979)}{93 -- 98}
  \end{article}
  \begin{article}{BuGo99}{Bux.Gonzalez:1999}
    \au{K-U.\nametie Bux, C.R.\nametie Gonzalez}
    \ti{The Bestvina-Brady Construction Revisited -- Geometric Computation
        of $\Sigma$-Invariants for Right Angled Artin Groups}
    \lo{Journal of the London Mathematical Society (2) 60 (1999)}{793 -- 801}
%    \url{http://www.math.utah.edu/\~{}bux/math/bugo97.ps.gz}
  \end{article}
  \begin{article}{Bux97a}{Bux:1997a}%
    \au{K.-U.\nametie Bux}
    \ti{Finiteness Properties of some Metabelian $S$-Arithmetic Groups}
    \lo{Proceedings of the London Mathematical Society 75 (1997)}{308 -- 322}
  \end{article}
  \begin{thesis}{Bux97b}{Bux:1997b}%
    \au{K.-U.\nametie Bux}
    \ti{{\selectlanguage{german}Endlichkeitseigenschaften auf"|l\"o{}sbarer
        arithmetischer Gruppen \"u{}ber Funktionenk\"o{}rpern}}
    \lo{PhD thesis (Frankfurt, 1997)}{}
%    \url{http://www.math.uni-frankfurt.de/\~{}bux/math/bux98.ps.gz}
  \end{thesis}
  \begin{article}{Bux02}{Bux:2002}
    \au{K-U.\nametie Bux}
    \ti{Finiteness Properties of Soluble Arithmetic Groups over Global
        Function Fields}
    \lo{Preprint (2002)}{}
%    \url{http://www.math.utah.edu/\~{}bux/math/bux99b.ps.gz}
  \end{article}
  \begin{article}{Bux99b}{Bux:1999b}
    \au{K.-U.\nametie Bux}
    \ti{Orbit spaces of subgroup complexes, Morse Theory, and a new proof of a conjecture of Webb}
    \lo{Topology Proceedings 24 (Spring 1999)}{39 -- 51}
  \end{article}
  \begin{article}{Bux99}{Bux:1999}
    \au{K.-U.\nametie Bux}
    \ti{Orbit spaces of subgroup complexes, Morse Theory, and a new proof of a conjecture of Webb}
    \lo{Topology Proceedings 24 (Spring 1999)}{39 -- 51}
  \end{article}
  \begin{preprint}{Bux01}{Bux:2001}
    \au{K.-U.\nametie Bux}
    \ti{Finiteness Properties of Soluble Arithmetic Groups -- a Survey}
    \lo{To appear in Proceedings ``Groups: Geometric and Combinatorial Aspects'' (Bielefeld, 1999)}{}
    \url{http://www.math.cornell.edu/\~{}bux/math/bux99d.ps.gz}
  \end{preprint}
  \begin{article}{Bux03a}{Bux:2003a}
    \au{K-U.\nametie Bux}
    \ti{Finiteness Properties of Soluble Arithmetic Groups over Global
        Function Fields}
    \lo{%
      Submitted to Geometry and Topology (2003)
      arXiv:math.GR/0212365}{}
%    \url{http://www.math.utah.edu/\~{}bux/math/bux99b.ps.gz}
  \end{article}
  \begin{preprint}{Bux03b}{Bux:2003b}
    \au{K.-U.\nametie Bux}
    \ti{Brading and Tangling the Chessboard Complex}
    \lo{Preprint, arXiv:math.GT/0310420}{}
  \end{preprint}
  \begin{article}{Cann87}{Cannon:1987}
    \au{J.W.\nametie Cannon}
    \ti{Almost convex groups}
    \lo{Geometriae Dedicata 22 (1987)}{197 -- 210}
  \end{article}
  \begin{article}{CFGT89}{Cannon.Floyd.Grayson.Thurston:1989}
    \au{J.W.\nametie Cannon, W.J.\nametie Floyd, M.A.\nametie Grayson, W.P.\nametie Thurston}
    \ti{Solvgroups are not Almost Convex}
    \lo{Geometria Dedicata 31 (1989)}{291 -- 300}
  \end{article}
  \begin{article}{CFP96}{Cannon.Floyd.Parry:1996}
    \au{J.W.\nametie Cannon, W.J.\nametie Floyd, W.R.\nametie Parry}
    \ti{Introductory Notes to Richard~Thompson's Groups}
    \lo{L'Enseignement Math\'{e}matique 42 (1996)}{215 -- 256}
  \end{article}
  \begin{book}{CaFr67}{Cassels.Froehlich:1967}
    \ed{J.W.S.\nametie Cassels, A.\nametie Fr\"o{}hlich}
    \ti{Algebraic Number Theory. Proceedings of an Instructional
        Conference organized by the London Mathematical Society
        (A Nato Advanced Study Institute)
        with Support of the International Mathematical Union}
    \lo{Academic Press, London (1967)}{}
   \end{book}
  \begin{article}{Chev60}{Chevalley:1960}%
    \au{C.\nametie Chevalley}
    \ti{{\selectlanguage{french}Certain Sch\'{e}mas de Groupes Semi-Simples}}
    \lo{{\selectlanguage{french}S\'{e}minaire Bourbaki 13e ann\'{e}e (1960/61) n$\circ$~219}}{1 -- 16}
  \end{article}
  \begin{article}{Chou80}{Chou:1980}
    \au{C.\nametie Chou}
    \ti{Elementary amenable groups}
    \lo{Illinois Journal of Mathematics 24 (1980)}{396 -- 407}
  \end{article}
  \begin{preprint}{ClTa02}{Cleary.Taback:2002}
    \au{S.\nametie Cleary, J.\nametie Taback}
    \ti{Thompson's Group $F$ is not Almost Convex}
    \lo{Preprint (2002), to appear: Journal of Algebra}{}
  \end{preprint}
  \begin{preprint}{ClTa03}{Cleary.Taback:2003}
    \au{S.\nametie Cleary, J.\nametie Taback}
    \ti{Seesaw Words in Thompson's Group $F$}
    \lo{Preprint (2003) arXiv:math.GR/0310466}{}
  \end{preprint}
  \begin{book}{CMNS99}{Cossey.Miller.Neumann.Shapiro:1999}
      \ed{J.\nametie Cossey, C.F.\nametie Miller, W.\nametie Neumann and M.\nametie Shapiro}
      \ti{Geometric Group Theory down under}
      \lo{Proc.\ of the special year on geometric group theory,
          Australia Nat.\ Univ.\ Canberra, 1996 (de Gruyter, 1999)}{}
  \end{book}
  \begin{article}{CuMo87}{Culler.Morgan:1987}
    \au{M.\nametie Culler, K.\nametie Vogtmann}
    \ti{Group Actions on $\RRR$-Trees}
    \lo{Proceedings of the London Mathematical Society 35 (1987)}{571 -- 604}
  \end{article}
  \begin{article}{CuVo86}{Culler.Vogtmann:1986}
    \au{M.\nametie Culler, K.\nametie Vogtmann}
    \ti{Moduli of graphs and automorphisms of free groups}
    \lo{Inventiones mathematicae 84 (1986)}{91 -- 119}
  \end{article}
  \begin{article}{DaSh91}{Davis.Shapiro:1991}
    \au{M.W.\nametie Davis, M.\nametie Shapiro}
    \ti{Coxeter Groups are Almost Convex}
    \lo{Geometria Dedicata 39 (1991)}{55 -- 57}
  \end{article}
  \begin{thesis}{Dege00}{Degenhardt:2000}
    \au{F.\nametie Degenhardt}
    \ti{{\selectlanguage{german}Endlichkeitseigenschaften gewisser
         Gruppen von Z\"{o}pfen unendlicher Ordnung}}
    \lo{PhD thesis (Frankfurt, 2000)}{}
  \end{thesis}
  \begin{book}{DiDu89}{Dicks.Dunwoody:1989}
    \au{W.\nametie Dicks, M.J.\nametie Dunwoods}
    \ti{Groups acting on graphs}
    \lo{Cambridge studies in advanced mathematics 17 (Cambridge University Press, 1989)}{}
  \end{book}
  \begin{article}{EiGa57}{Eilenberg.Ganea:1957}
    \au{S.\nametie Eilenberg, T.\nametie Ganea}
    \ti{On the Lusternik-Schnirelmann category of abstract groups}
    \lo{Annals of Mathematics 65 (1957)}{517 -- 518}
  \end{article}
  \begin{book}{Eggl58}{Eggleston:1958}%
    \au{H.G.\nametie Eggleston}
    \ti{Convexity}
    \lo{Cambridge Tracts in Mathematics and Mathematical Physics, Cambridge (1958)}{}
  \end{book}
  \begin{preprint}{ElHe02}{Elder.Hermiller:2002}
    \au{M.\nametie Elder, S.\nametie Hermiller}
    \ti{Minimal almost convexity: some examples.}
    \lo{in preparation}{}
  \end{preprint}
  \begin{article}{Epst62}{Epstein:1962}
    \au{D.B.A.\nametie Epstein}
    \ti{Ends}
    \lo{in \cite{Fort:1962}}{110 -- 117}
  \end{article}
  \begin{article}{FaNe62}{Fadell.Neuwirth:1962}
    \au{E.\nametie Fadell, L.\nametie Neuwirth}
    \ti{Configuration Spaces}
    \lo{Mathematica Scandinavica 10 (1962)}{111 -- 118}
  \end{article}
  \begin{thesis}{Ford95}{Fordham:1995}
    \au{S.B.\nametie Fordham}
    \ti{Minimal Length Elements of Thompson's Group $F$}
    \lo{PhD Thesis (Brigham Young University, 1995)}{}
  \end{thesis}
  \begin{article}{For98a}{Forman:1998a}
    \au{R.\nametie Forman}
    \ti{Morse theory for cell complexes}
    \lo{Advances in Mathematics 134 (1998)}{90 -- 145}
  \end{article}
  \begin{article}{For98b}{Forman:1998b}
    \au{R.\nametie Forman}
    \ti{Witten-Morse theory for cell complexes}
    \lo{Topology 37 (1998)}{945 --979}
  \end{article}
  \begin{book}{Fort62}{Fort:1962}%
    \ed{M.K.\nametie Fort}
    \ti{Topology of 3-Manifolds}
    \lo{Proceedings of The University of Georgia Institute (1961), Prentice-Hall 1962}{}
  \end{book}
  \begin{book}{GHV90}{Ghys.Haefliger.Verjovsky:1990}%
    \ed{E.\nametie Ghys, A.\nametie Haefliger, A.\nametie Verjovsky}
    \ti{Groups from a geometric viewpoint}
    \lo{Proceedings of the workshop held in Trieste, March 26--April 6, 1990}{World Sci. Publishing, 1991}
  \end{book}
  \begin{article}{Grig80}{Grigorchuk:1980}
    \au{R.I.\nametie Grigorchuk}
    \ti{On Burnside's Problem on periodic groups}
    \lo{Functional Analysis Applications 14 (1980)}{41 -- 43}
  \end{article}
  \begin{article}{Grig83}{Grigorchuk:1983}
    \au{R.I.\nametie Grigorchuk}
    \ti{On the Milnor problem of group growth}
    \lo{Dokl. Akad. Nauk. SSSR 271 (1983)}{30 -- 33}
  \end{article}
  \begin{article}{Grig84}{Grigorchuk:1984}
    \au{R.I.\nametie Grigorchuk}
    \ti{Degrees of growth of finitely generated groups and the theory of
        invariant means. (Russian)}
    \lo{Izv. Akad. Nauk SSSR Ser. Mat. 48 (1984), no. 5}{939 -- 985}
  \end{article}
  \begin{article}{Grig85}{Grigorchuk:1985}
    \au{R.I.\nametie Grigorchuk}
    \ti{On the growth degrees of $p$-groups and torsion free groups}
    \lo{Math. USSR Sbornik 54 (1986)}{185 -- 205}
  \end{article}
  \begin{article}{Gri98}{Grigorchuk:1998}
    \au{R.I.\nametie Grigorchuk}
    \ti{An example of a finitely presented amenable group not belonging to the class $EG$}
    \lo{Math. USSR Sbornik 189 (1998)}{75 -- 95}
  \end{article}
  \begin{article}{GrWi00}{Grigorchuk.Wilson:2000}
    \au{R.I.\nametie Grigorchuk, J.S.\nametie Wilson}
    \ti{The Conjugacy Problem for Certain Branch Groups}
    \lo{Proceedings of the Steklov Institute of Mathematics 231 (2000)}{204 -- 219}
  \end{article}
  \begin{article}{Grom81}{Gromov:1981}
    \au{M.\nametie Gromov}
    \ti{Groups of Polynomial Growth and Expanding Maps}
    \lo{Publicationes Mathematicae IHES 53 (1981)}{53 -- 73}
  \end{article}
  \begin{book}{GrRo84}{Gruenberg.Roseblade:1984}
    \ed{K.W.\nametie Gruenberg, J.E.\nametie Roseblade}
    \ti{Group Theory: Essays for Philip Hall}
    \lo{Academic Press (1984)}{}
  \end{book}
  \begin{article}{Grus40}{Grushko:1940}
    \au{I.A.\nametie Grushko}
    \ti{{\selectlanguage{german}^^dcber die Basen eines freien Produktes von Gruppen} (Russian, with German summary)}
    \lo{Mat. Sb. 8 (1940)}{169 -- 182}
  \end{article}
  \begin{preprint}{Guba02a}{Guba:2002a}
    \au{V.S.\nametie Guba}
    \ti{The Dehn Function of Richard Thompson's Group $F$ is Quadratic}
    \lo{Preprint (2002), arXiv:math.GR/0211395 v1}{}
  \end{preprint}
  \begin{preprint}{Guba02}{Guba:2002b}
    \au{V.S.\nametie Guba}
    \ti{On the Properties of the Cayley Graph of Richard Thompson's Group $F$}
    \lo{Preprint (2002), arXiv:math.GR/0211396 v1}{}
  \end{preprint}
  \begin{book}{GuSa97}{Guba.Sapir:1997}
    \au{V.S.\nametie Guba, M.S.\nametie Sapir}
    \ti{Diagram Groups}
    \lo{Mem. Amer. Math. Soc. 130 (1997)}{}
  \end{book}
  \begin{article}{GuSa99}{Guba.Sapir:1999}
    \au{V.S.\nametie Guba, M.V.\nametie Sapir}
    \ti{On subgroups of the R. Thompson group $F$ and other diagram groups}
    \lo{Math. USSR Sbornik 190 (1999), no. 7-8}{1077--1130}
   \end{article}
  \begin{article}{Hare85}{Harer:1985}
    \au{J.L.\nametie Harer}
    \ti{Stability of the homology of the mapping class groups of orientable surfaces}
    \lo{Annals of Mathematics 121 (1985)}{215 -- 249}
  \end{article}
  \begin{article}{Hare86}{Harer:1986}
    \au{J.L.\nametie Harer}
    \ti{The virtual cohomological dimension of the mapping class group of an orientable surface.}
    \lo{Inventiones mathematicae 84 (1986)}{157 -- 176}
  \end{article}
  \begin{article}{Harv79}{Harvey:1979}
    \au{W.J.\nametie Harvey}
    \ti{Geometric structure of surface mapping class groups}
    \lo{In \cite{Wall:1979}}{255 -- 269}
  \end{article}
  \begin{article}{HaMe96}{Harlander.Meinert:1996}
    \au{J.\nametie Harlander, H.\nametie Meinert}
    \ti{Higher generation subgroup sets and the virtual cohomological dimension of graph
      products of finite groups}
    \lo{Journal of the London Mathematical Society 53 (1996)}{99 -- 117}
  \end{article}
  \begin{book}{Harp00}{Harpe:2000}
    \au{P.\nametie de~la~Harpe}
    \ti{Topics in Geometric Group Theory}
    \lo{University of Chicago Press (2000)}{}
  \end{book}
  \begin{book}{Hat01}{Hatcher:2001}
    \au{A.\nametie Hatcher}
    \ti{Algebraic Topology}
    \lo{Cambridge University Press (2001)}{}
    \www{http://www.math.cornell.edu/\~{}hatcher/AT/ATpage.html}
  \end{book}
  \begin{article}{HaVo96}{Hatcher.Vogtmann:1996}
    \au{A.\nametie Hatcher, K.\nametie Vogtmann}
    \ti{Isoperimetric Inequalities for Automorphism Groups of Free Groups}
    \lo{Pacific Journal of Mathematics 173 (1996)}{425 -- 441}
  \end{article}
  \begin{preprint}{Heyd99}{Heydebreck:1999}
    \au{A.\nametie von~Heydebreck}
    \ti{Homotopy properties of certain complexes associated to spherical buildings}
    \lo{Preprint, (Frankfurt 1999)}{}
  \end{preprint}
  \begin{report}{Higm74}{Higman:1974}
    \au{G.\nametie Higman}
    \ti{Finitely Presented Infinite Simple Groups}
    \lo{Australian Nat.\ University, Notes in Pure Mathematics 8 (Canberra, 1974)}{}
  \end{report}
  \begin{article}{Hows54}{Howson:1954}
    \au{A.G.\nametie Howson}
    \ti{On the intersection of finitely generated free groups}
    \lo{Journal of the London Mathematical Society 29 (1954)}{428 -- 434}
  \end{article}
  \begin{article}{Inci97}{Incitti:1997}
    \au{R.\nametie Incitti}
    \ti{Regularities on the Cayley Graphs of Groups of Linear Growth}
    \lo{European Journal of Combinatorics 18 (1997)}{175 -- 178}
  \end{article}
  \begin{article}{Ivan97}{Ivanov:1997}
    \au{N.V.\nametie Ivanov}
    \ti{Automorphisms of complexes of curves and of Teichm^^fcller spaces}
    \lo{International Mathematical Research Notices (1997) no. 14}{651 - 666}
  \end{article}
  \begin{article}{John83}{Johnson:1983}
    \au{D.\nametie Johnson}
    \ti{The structure of the Torelli group I: A finite set of generators for $\mathcal{J}$}
    \lo{Annals of Mathematics 118 (1983)}{423 -- 442}
  \end{article}
  \begin{article}{Kapo02}{Kapovich:2002}
    \au{I.\nametie Kapovich}
    \ti{A note on the Po\'{e}naru condition}
    \lo{Journal of Group Theory 5 (2002)}{119 -- 127}
  \end{article}
  \begin{manuscript}{Kirb95}{Kirby:1995}
    \au{R.\nametie Kirby}
    \ti{Problems in Low-Dimensional Topology}
    \lo{Manuskript (Berkeley, 1995)}{}
    \www{http://www.math.berkeley.edu/\~{}kirby/}
  \end{manuscript}
  \begin{article}{KM98a}{Kharlampovic.Myasnikov:1998a}
    \au{O.\nametie Kharlampovic, A.\nametie Myasnikov}
    \ti{Tarski's problem about the elementary theory of free groups has a positive
      solution}
    \lo{ERA-AMS (1998)}{101 -- 108}
  \end{article}
  \begin{article}{KM98b}{Kharlampovic.Myasnikov:1998b}
    \au{O.\nametie Kharlampovic, A.\nametie Myasnikov}
    \ti{Irreducible affine varieties over a free group. I: Irreducibility of quadratic
      equations and Nullstellensatz} % (paper 1 on the theory of a free group)
    \lo{Journal of Algebra 200 (1998)}{472 -- 516}
  \end{article}
  \begin{article}{KM98c}{Kharlampovic.Myasnikov:1998c}
    \au{O.\nametie Kharlampovic, A.\nametie Myasnikov}
    \ti{Irreducible affine varieties over a free group. II: Systems in row-echelon form
      and description of residually free groups} % (paper 2 on the theory of a free group)
    \lo{Journal of Algebra 200,(1998)}{517 -- 570}
  \end{article}
  \begin{article}{KM00a}{Kharlampovic.Myasnikov:2000a}
    \au{O.\nametie Kharlampovic, A.\nametie Myasnikov}
    \ti{Implicit function theorem over free groups}
    \lo{preprint}{}
  \end{article}
  \begin{article}{KM00b}{Kharlampovic.Myasnikov:2000b}
    \au{O.\nametie Kharlampovic, A.\nametie Myasnikov}
    \ti{Equations over fully residually free groups}
    \lo{preprint}{}
  \end{article}
  \begin{article}{KM00c}{Kharlampovic.Myasnikov:2000c}
    \au{O.\nametie Kharlampovic, A.\nametie Myasnikov}
    \ti{Elementary theory of free nonabelian groups}
    \lo{preprint}{}
  \end{article}
  \begin{article}{Knes64}{Kneser:1964}%
    \au{M.\nametie Kneser}
    \ti{{\selectlanguage{german}Erzeugende und Relationen verallgemeinerter Einheitengruppen}}
    \lo{{\selectlanguage{german}Journal f\"u{}r die Reine und Angewandte Mathematik} 214/215 (1964)}{345 -- 349}
  \end{article}
  \begin{thesis}{Koch97}{Kochloukova:1997}
    \au{D.\nametie Kochloukova}
    \ti{The FP${}^m$-Conjecture for a class of metabelian groups}
    \lo{PhD thesis (Cambridge, 1997)}{}
  \end{thesis}
  \begin{thesis}{Kram95}{Krammer:1995}
    \au{D.\nametie Krammer}
    \ti{The conjugacy problem for Coxeter groups}
    \lo{PhD thesis (Utrecht 1995)}{}
  \end{thesis}
  \begin{article}{KMcC97}{Kristic.McCool:1997}
    \au{S.\nametie Kristi\'{c}, J.\nametie McCool}
    \ti{The non-finite presentability of $IA(F_3)$ and $\GL_2(\mathrm{Z}[t,t^{-1}])$}
    \lo{Inventiones mathematicae 129 (1997)}{595 -- 606}
  \end{article}
  \begin{book}{LSch77}{Lyndon.Schupp:1977}
    \au{R.C.\nametie Lyndon, P.E.\nametie Schupp}
    \ti{Combinatorial Group Theory}
    \lo{{\selectlanguage{german}Ergebnisse der Mathematik und ihrer Grenzgebiete 89} (Springer, 1977)}{}
  \end{book}
  \begin{article}{Lys85}{Lysenok:1985}
    \au{I.G.\nametie Lysenok}
    \ti{A System of Defining Relations for a Grigorchuk Group}
    \lo{Translations: Matematicheskie Zametki 38 (1985)}{784 -- 792}
  \end{article}
  \begin{article}{Macb64}{Macbeath:1964}%
    \au{A.M.\nametie Macbeath}
    \ti{Groups of homeomorphisms of a simply connected space}
    \lo{Annals of Math 79 (1964)}{473--488}
  \end{article}
  \begin{article}{Magn34}{Magnus:1934}
    \au{W.\nametie Magnus}
    \ti{{\selectlanguage{german}^^dcber $n$-dimensionale Gittertransformationen}}
    \lo{Acta mathematica 64 (1934)}{353 -- 367}
  \end{article}
  \begin{book}{Magn74}{Magnus:1974}
    \au{W.\nametie Magnus}
    \ti{Noneuclidean Tesselations and their Groups}
    \lo{Academic Press (New York, London 1974)}{}
  \end{book}
  \begin{article}{Maka82}{Makanin:1982}
    \au{G.S.\nametie Makanin}
    \ti{Equations in a Free Group}
    \lo{Math. USSR Izvestiya 21 (1983)}{483 -- 546}
  \end{article}
  \begin{article}{McCM86}{McCullough.Miller:1986}
    \au{D.\nametie McCullough, A.\nametie Miller}
    \ti{The genus $2$ Torelli group is not finitely generated}
    \lo{Topology Applications 22 (1986) no.\ 1}{43 -- 49}
  \end{article}
  \begin{article}{Mess92}{Mess:1992}
    \au{G.\nametie Mess}
    \ti{The Torelli groups for genus $2$ and $3$ surfaces}
    \lo{Topology 31 (1992) no. 4}{775 -- 790}
  \end{article}
  \begin{article}{Meie82}{Meier:1982}
    \au{D.\nametie Meier}
    \ti{Non-Hopfian Groups}
    \lo{Journal of the London Mathematical Society 26 (1982)}{265 -- 270}
  \end{article}
  \begin{article}{MMV98}{Meier.Meinert.VanWyk:1998}
    \au{J.\nametie Meier, H.\nametie Meinert, L.\nametie VanWyk}
    \ti{Higher generation subgroup sets and the $\Sigma$-invariants of graph groups}
    \lo{Commentarii Mathematici Helvetici 73 (1998)}{22 -- 44}
  \end{article}
  \begin{article}{Mein96}{Meinert:1996}%
    \au{H.\nametie Meinert}
    \ti{The homological invariants for metabelian groups of
        finite Pr\"u{}fer rank: a proof of the $\Sigma^m$-conjecture}
    \lo{Proceedings of the London Mathematical Society 72 (1996)}{385 -- 424}
  \end{article}
  \begin{article}{Mein97}{Meinert:1997}%
    \au{H.\nametie Meinert}
    \ti{Actions on $2$-complexes and the homotopical invariant
        $\Sigma^2$ of a group}
    \lo{Journal of Pure and Applied Algebra 119 (1997)}{297 -- 317}
  \end{article}
  \begin{thesis}{Mein93}{Meinert:1993}%
    \au{H.\nametie Meinert}
    \ti{{\selectlanguage{german}Die h\"o{}heren geometrischen Invarianten~$\Sigma^m$ von Gruppen
        via Operationen auf CW-Komplexen und der Beweis der
        $\Sigma^m$-Vermutung f\"u{}r metabelsche Gruppen endlichen
        Pr\"u{}fer-Ranges}}
    \lo{PhD thesis (Frankfurt, 1993)}{}
  \end{thesis}
  \begin{article}{MiSh98}{Miller.Shapiro:1998}
    \au{C.F.\nametie Miller~III, M.\nametie Shapiro}
    \ti{Solvable Baumslag-Solitar Groups are not Almost Convex}
    \lo{Geometria Dedicata 72 (1998)}{123 -- 127}
  \end{article}
  \begin{book}{Miln99}{Milnor:1999}
    \au{J.W.\nametie Milnor}
    \ti{Dynamics in One Complex Variable}
    \lo{Vieweg (1999)}{}
  \end{book}
  \begin{book}{Mois77}{Moise:1977}
    \au{E.E.\nametie Moise}
    \ti{Geometric Topology in Dimensions 2 and 3}
    \lo{Springer GTM 47}{}
  \end{book}
  \begin{preprint}{Nekr03}{Nekrashevych:2003}
    \au{V.\nametie Nekrashevich}
    \ti{Iterated Monodromy Groups}
    \lo{perprint (2003) arXiv:math.DS/0312306}{}
  \end{preprint}
  \begin{article}{Neum37}{Neumann:1937}%
    \au{B.H.\nametie Neumann}
    \ti{Some remarks on infinite groups}
    \lo{Journal of the London Mathematical Society 12 (1937)}{120 -- 127}
  \end{article}
  \begin{article}{Neum55}{Neumann:1955}
    \ti{On the intersection of finitely generated free groups}
    \au{H.\nametie Neumann}
    \lo{Publ. Math. Debrecen 4 (1955-56)}{186 -- 189}
    [\lo{Addendum: ibid. 5 (1957-58)}{128}]
  \end{article}
  \begin{article}{Nosk97}{Noskov:1997}
    \au{G.A.\nametie Noskov}
    \ti{The Bieri-Strebel invariant and homological finiteness conditions for metabelian groups}
    \lo{Algebra and Logic 36 (1997)}{117 -- 132}
  \end{article}
  \begin{book}{O'Me73}{OMeara:1973}%
    \au{O.T.\nametie O'Meara}
    \ti{Introduction to Quadratic Forms}
    \lo{Berlin, Heidelberg, New~York (Springer, 1973)}{}
  \end{book}
  \begin{thesis}{Prov77}{Provan:1977}
    \au{J.S.\nametie Provan}
    \ti{Decopositions, shellings and diameters of simplicial complexes and convex polytopes}
    \lo{Thesis, Cornell University (1977)}{}
  \end{thesis}
  \begin{article}{Quil78}{Quillen:1978}
    \au{D.\nametie Quillen}
    \ti{Homotopy Properties of the Poset of Nontrivial $p$-Subgroups of a Group}
    \lo{Advances in Mathematics 28 (1978)}{101 -- 128}
  \end{article}
  \begin{article}{Ragh68}{Raghunatan:1968}
    \au{M.S.\nametie Raghunatan}
    \ti{A Note on Quotients of Real Algebraic Groups by Arithmetic Subgroups}
    \lo{Inventiones mathematicae 4 (1968)}{318 -- 335}
  \end{article}
  \begin{article}{Razb84}{Razborov:1984}
    \au{A.A.\nametie Razborov}
    \ti{On Systems of Equations in a Free Group}
    \lo{Math. USSR Izvestiya 25 (1985)}{115 -- 162}
  \end{article}
  \begin{thesis}{Renz88}{Renz:1988}
    \au{B.\nametie Renz}
    \ti{{\selectlanguage{german}Geometrische Invarianten und Endlichkeitseigenschaften von
        Gruppen}}
    \lo{PhD thesis (Frankfurt, 1988)}{}
  \end{thesis}
  \begin{preprint}{Rile02}{Riley:2002}
    \au{T.R.\nametie Riley}
    \ti{The geometry of groups satisfying weak almost-convexity or weak geodesic-combability conditions}
    \lo{Journal of Group Theory 5 (2002)}{513 -- 525}
  \end{preprint}
  \begin{book}{Rona89}{Ronan:1989}%
    \au{M.\nametie Ronan}
    \ti{Lectures on Buildings}
    \lo{Perspectives in Mathematics,
        Academic Press, San~Diego, London (1989)}{}
  \end{book}
  \begin{article}{SBR02}{Birget.Sapir.Rips:2002}
    \au{M.V.\nametie Sapir, J.C.\nametie Birget, E.\nametie Rips}
    \ti{Isoperimetric and Isodiametric Functions of Groups}
    \lo{Annals of Mathematics 156 (2002)}{345 -- 466}
  \end{article}
  \begin{article}{Salv94}{Salvetti:1994}
    \au{M.\nametie Salvetti}
    \ti{The Homotopy Type of Artin Groups}
    \lo{Mathematical Research Letters 1 (1994)}{565 -- 577}
  \end{article}
  \begin{article}{Se01a}{Sela:2001a}%
    \au{Z.\nametie Sela}
    \ti{Diphantine Geometry over Groups I: Makanin-Razborov diagrams}
    \lo{preprint}{}
  \end{article}
  \begin{article}{Se01b}{Sela:2001b}%
    \au{Z.\nametie Sela}
    \ti{Diphantine Geometry over Groups  II: Completions, closures and formal solutions}
    \lo{preprint}{}
  \end{article}
  \begin{article}{Se01c}{Sela:2001c}%
    \au{Z.\nametie Sela}
    \ti{Diphantine Geometry over Groups III: Rigid and solid solutions}
    \lo{preprint}{}
  \end{article}
  \begin{article}{Se01d}{Sela:2001d}%
    \au{Z.\nametie Sela}
    \ti{Diphantine Geometry over Groups IV: An iterative procedure for validation of a sentence}
    \lo{preprint}{}
  \end{article}
  \begin{article}{Se01e}{Sela:2001e}%
    \au{Z.\nametie Sela}
    \ti{Diphantine Geometry over Groups  V: Quantifier elimination}
    \lo{preprint}{}
  \end{article}
  \begin{article}{Se01f}{Sela:2001f}%
    \au{Z.\nametie Sela}
    \ti{Diphantine Geometry over Groups VI: The elementary theory of a free group}
    \lo{preprint}{}
  \end{article}
  \begin{book}{Serr77}{Serre:1977}%
    \au{J.-P.\nametie Serre}
    \ti{{\selectlanguage{french}Arbres, amalgames, $SL_2$}}
    \lo{Asterique 46 (1977)}{}
  \end{book}
  \begin{article}{Serr79}{Serre:1979}
    \au{J.P.\nametie Serre}
    \ti{Arithmetic Groups}
    \lo{In \cite{Wall:1979}}{105 -- 136}
  \end{article}
  \begin{article}{ShSt95}{Shapiro.Stein:1995}
    \au{M.\nametie Shapiro, M.I.\nametie Stein}
    \ti{Almost Convex Groups and the Eight Geometries}
    \lo{Geometria Dedicata 55 (1995)}{125 -- 140}
  \end{article}
  \begin{article}{Shor90}{Short:1990}
    \au{H.\nametie Short}
    \ti{Quasiconvexity and a Theorem of Howson}
    \lo{in \cite{Ghys.Haefliger.Verjovsky:1990}}{168 -- 176}
  \end{article}
  \begin{preprint}{Skor??}{Skora:unknown}
    \au{R.\nametie Skora}
    \ti{Deformation of Length Functions in Groups}
    \lo{Preprint (????)}{}
  \end{preprint}
  \begin{article}{Smal57}{Smale:1957}
    \au{S.\nametie Smale}
    \ti{A Vietoris Mapping Theorem for Homotopy}
    \lo{Proceedings of the American Mathematical Society 8 (1957)}{604 -- 610}
  \end{article}
  \begin{article}{SV87a}{Smillie.Vogtmann:1987a}
    \au{J.\nametie Smillie, K.\nametie Vogtmann}
    \ti{A Generating Function for the Euler Characteristic of Out$(F_n)$}
    \lo{Journal of Pure and Applied Algebra 44 (1987)}{329 -- 348}
  \end{article}
  \begin{article}{SV87b}{Smillie.Vogtmann:1987b}
    \au{J.\nametie Smillie, K.\nametie Vogtmann}
    \ti{Automorphisms of Graphs, $p$-subgroups of Out$(F_n)$ and the Euler Characteristic of Out$(F_n)$}
    \lo{Journal of Pure and Applied Algebra 49 (1987)}{182 -- 200}
  \end{article}
  \begin{book}{Span66}{Spanier:1966}
    \au{E.H.\nametie Spanier}
    \ti{Algebraic Topology}
    \lo{Springer, New York (1966)}{}
  \end{book}
  \begin{article}{Stal68}{Stallings:1968}
    \au{J.R.\nametie Stallings}
    \ti{On torsion-free groups with infinitely many ends}
    \lo{Annals of Mathematics 88 (1968)}{312 -- 334}
  \end{article}
  \begin{article}{Stal88}{Stallings:1988}
    \au{J.\nametie Stallings}
    \ti{Foldings of $G$-trees}
    \lo{in \cite{Alperin:1991}}{355 -- 368}
  \end{article}
  \begin{notes}{Stei68}{Steinberg:1968}%
    \au{R.\nametie Steinberg}
    \ti{Lectures on Chevalley Groups,
        Notes prepared by John Faulkner and Robert Wilson.}
    \lo{Yale University, New Haven, Connecticut, (1968)}{}
  \end{notes}
  \begin{article}{Stre84}{Strebel:1984}%
    \au{R.\nametie Strebel}
    \ti{Finitely Presented Solvable Groups}
    \lo{In \cite{Gruenberg.Roseblade:1984}}{257 -- 314}
  \end{article}
  \begin{article}{Stuh76}{Stuhler:1976}%
    \au{U.\nametie Stuhler}
    \ti{{\selectlanguage{german}Zur Frage der endlichen Pr\"a{}sentiertheit gewisser
        arithmetischer Gruppen im Funktionenk\"o{}rperfall}}
    \lo{{\selectlanguage{german}Mathematische Annalen 224 (1976)}}{217 -- 232}
  \end{article}
  \begin{article}{Stuh80}{Stuhler:1980}%
    \au{U.\nametie Stuhler}
    \ti{Homological properties of certain arithmetic groups in
        the function field case}
    \lo{Inventiones mathatematicae 57 (1980)}{263 -- 281}
  \end{article}
  \begin{article}{Symo98}{Symonds:1998}%
    \au{P.\nametie Symonds}
    \ti{The orbit space of the $p$-subgroup complex is contractible}
    \lo{Commentarii Mathematici Helvetici 73 (1998)}{400 -- 405}
  \end{article}
  \begin{thesis}{Tiem94}{Tiemeyer:1994}%
    \au{A.\nametie Tiemeyer}
    \ti{{\selectlanguage{german}Kompaktheitseigenschaften lokalkompakter Gruppen}}
    \lo{PhD thesis (Bielefeld, 1994)}{}
  \end{thesis}
  \begin{article}{Tiem97}{Tiemeyer:1997}%
    \au{A.\nametie Tiemeyer}
    \ti{A Local-Global Principle for Finiteness Properties of
      $S$-Artihmetic Groups over Number Fields}
    \lo{Transformation Groups 2 (1997)}{215 -- 223}
%    (confere~\cite{Abels.Tiemeyer:1997})
  \end{article}
  \begin{article}{Tits72}{Tits:1972}%
    \au{J.\nametie Tits}
    \ti{Free Subgroups in Linear Groups}
    \lo{Journal of Algebra 20 (1972)}{250 -- 270}
  \end{article}
  \begin{article}{Tits87}{Tits:1987}%
    \au{J.\nametie Tits}
    \ti{Uniqueness and Presentations of Kac-Moody Groups over Fields}
    \lo{Journal of Algebra~105 (1987)}{542 -- 573}
  \end{article}
  \begin{article}{Vogt90}{Vogtmann:1990}
    \au{K.\nametie Vogtmann}
    \ti{Local Structure of some $\mathop{\mathrm{OUT}}(F_n)$-Complexes}
    \lo{Proceedings of the Edinburgh Mathematical Society (1990)}{367 -- 379}
  \end{article}
  \begin{preprint}{Vogt00}{Vogtmann:2000}
    \au{K.\nametie Vogtmann}
    \ti{Automorphisms of Free Groups and Outer Space}
    \lo{To appear in the special issue of Geometriae Dedicata for the June, 2000 Haifa Conference
        on Geometric Group Theory}{}
  \end{preprint}
  \begin{article}{Wall65}{Wall:1965}
    \au{C.T.C.\nametie Wall}
    \ti{Finiteness Conditions for CW-Complexes}
    \lo{Annals of Mathematics 81 (1965)}{56 -- 69}
  \end{article}
  \begin{book}{Wall79}{Wall:1979}
    \ed{C.T.C.\nametie Wall}
    \ti{Homological Group Theory}
    \lo{LMS Lecture Notes 35, Cambridge University Press (Cambridge 1979)}{}
  \end{book}
  \begin{book}{Weil73}{Weil:1973}%
    \au{A.\nametie Weil}
    \ti{Basic Number Theory}
    \edition{Reprint of the Second Edition (1973)}
    \lo{Springer Classics in Mathematics, Berlin Heidelberg (1995)}{}
  \end{book}
  \begin{book}{Whit92}{White:1992}
    \ed{N.\nametie White}
    \ti{Matroid Applications, volume 40 of Encyclopedia of Mathematics}
    \lo{Cambridge University Press (1992)}{}
  \end{book}
\end{references}
\endinput

